Ancient Coin Classification Using Graph Transduction Games

Recognizing the type of an ancient coin requires theoretical expertise and years of experience in the field of numismatics. Our goal in this work is automatizing this time consuming and demanding task by a visual classification framework. Specifically, we propose to model ancient coin image classification using Graph Transduction Games (GTG). GTG casts the classification problem as a non-cooperative game where the players (the coin images) decide their strategies (class labels) according to the choices made by the others, which results with a global consensus at the final labeling. Experiments are conducted on the only publicly available dataset which is composed of 180 images of 60 types of Roman coins. We demonstrate that our approach outperforms the literature work on the same dataset with the classification accuracy of 73.6% and 87.3% when there are one and two images per class in the training set, respectively.

==> bkg.tex <==



\\


%Similarity values are stored in matrix $W$.


==> gtg.tex <==
%%%%%% START COPYPASTE ICPR %%%%%%%%%%
Graph Transduction (GT) is a subfamily of semi-supervised learning that aims to classify unlabeled objects starting from a small set of labeled ones. In particular, in GT the data is modeled as a graph whose vertices are the objects in a dataset. The provided label information is then propagated all over the unlabeled objects through the edges, weighted according to the consistency of object pairs. The reader is encouraged to refer to \cite{ZhuSemiSupervised} for a detailed description of algorithms and applications on graph transduction.

%\begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth,trim={2.8cm 0.5cm 2.4cm 0.5cm},clip]{./figures/gtg.pdf}
%\vspace{-0.5cm}
% \caption{The dynamics of the GTG. The algorithm takes in input similarities between objects and hard/soft labelings of the object themselves. After three iterations, the algorithm has converged, generating a pseudo-label with 100\% confidence.}
%\vspace{-0.5cm}
%\end{figure}

More formally, let $G = (V, E, w)$ be a graph. $V$ is the vertex set of the objects and can be partitioned in two sets: $L = \{(f_1, y_1), ..., (f_l, y_l)\}$ contains the labeled objects, where $f_i \in \mathbb{R}^d$ is a real-valued vector describing the object (features), and $y_i \in \{1, 2...,m\}$ is its associated label, while $U = \{f_{l+1},...,f_{n}\}$ is the set of unlabeled objects. $E$ is the set of edges connecting the vertices and $w: E \rightarrow \mathbb{R}_{\geq 0}$ is a weight function that assigns a non-negative similarity measure to each edge in $E$, and can be summarized in a pairwise weight matrix $W$.

%In \cite{ZhuSemiSupervised}, GT takes in input $W$ along with initial probability distributions for every objects -- one-hot labels for $(f_i, y_i) \in L$, soft labels for $f_i \in U$ -- and iteratively applies a function $P: \Delta^m \rightarrow \Delta^m$ where $\Delta^m$ is the standard simplex. At each iteration, if the distributions of labeled objects have changed, they are reset. Once the algorithm reaches the convergence, the resulting final probabilities give a labeling over the entire set of objects.

In this article, we follow the approach proposed in \cite{DBLP:journals/neco/ErdemP12}, where the authors interpret the graph transduction task as a non-cooperative multiplayer game. The same methodology has been successfully applied in different context, e.g. bioinformatics \cite{DBLP:journals/jmiv/vascon2018} and label augmentation problem \cite{elezi2018transductive}.

In the graph transduction game (GTG), objects of a dataset are represented as players and their labels as strategies. In synthesis, a non-cooperative multiplayer game is played among the objects, until an equilibrium condition is reached, the \emph{Nash Equilibria} \cite{Nash1951}. 
Here, we provide some basic knowledge on game theory in order to be self-contained. Given a set of players $I = \{1, \dots, n\}$ and a set of possible pure strategies $S = \{1, \dots, m\}$:

\begin{enumerate}
\item \emph{mixed strategy}: a mixed strategy $x_i$ is a probability distribution over the possible strategies for player $i$. Then $x_i \in \Delta^m$, where 
$\Delta^m = \left\lbrace \sum_{h = 1}^{m} x_i(h) = 1, x_i(h) \geq 0, \ h = \{1, \dots, m\} \right\rbrace $
is the standard $m$-dimensional simplex and $x_i(h)$ is the probability of player $i$ choosing the pure strategy $h$.
\item \emph{mixed strategy space}: it corresponds to the set of all mixed strategies of the players
$x = \left\lbrace x_1, \dots, x_n \right\rbrace$
\item \emph{utility function}: it represents the gain obtained by a player when it chooses a certain mixed strategy, in particular $u: \Delta^m \rightarrow \mathbb{R}_{\geq 0}$.
\end{enumerate}
Here, it is assumed that the payoffs associated to each player are additively separable, thus the algorithm is a member of polymatrix games\cite{howson1972equilibria}.

In GTG, the aforementioned definitions turns into the following:
\paragraph{Strategy space} The strategy space $x$ is the starting point of the game and contains all the mixed strategies. The space $x$ can be initialized in different ways based on the fact that some prior knowledge exists or not. Here, we distinguish the initialization based on the type of object, \emph{labeled} or \emph{unlabeled}.
For the labeled object, since their class is known, a one-hot vector is assigned:
\begin{equation}\label{eq:Xprior}
x_i(h)=
\begin{cases}
	1, & \text{if } i \text{ has label } h \\
    0, & \text{ otherwise}.
\end{cases}
\end{equation}
For the unlabeled objects all the labels have the same probability of being associated to an object, thus:
\begin{equation}
x_i(h) = \frac{1}{m} \quad \text{ } h = \{1, \dots, m \}\label{eq:Xnoprior}
\end{equation}

\paragraph{Payoff function} 
The utility function reflects the likelihood of choosing a particular label and considers the similarity between labeled and unlabeled players. Similar players influence each other more in picking one of the possible strategies (labels). Once the game reaches an equilibrium, every player play their best strategies  which correspond to a consistent labeling \cite{miller1991copositive} not only for the player itself but also for the others.
Under equilibrium conditions the label of player $i$ is given by the strategy played with the highest probability. 

Formally, given a player $i$ and a strategy $h$:
\begin{eqnarray}
u_i(h)=\sum_{j \in U}{(A_{ij}x_j)_h}+\sum_{k=1}^{m}{\sum_{j \in L}{A_{ij}(h,k)}} \\
u_i(x)=\sum_{j \in U}{x_i^TA_{ij}x_j}+\sum_{k=1}^{m}{\sum_{j \in L}{x_i^T(A_{ij})_k}}
\end{eqnarray}
where $u_i(x)$ is the utility received by player $i$ when it plays the mixed strategy $x_i$ and $A_{ij} \in \mathbb{R}^{m \times m}$ is the \emph{partial payoff matrix} between players $i$ and $j$. As in \cite{DBLP:journals/neco/ErdemP12}, 
$A_{ij} = I_m \times \omega_{ij}$ where $\omega_{ij}$ is the similarity between player $i$ and $j$ and $I_m$ is the identity matrix of size $m \times m$.
The similarity function between players (objects) can be given or computed starting from the features. Given two objects $i, j$ and their features $f_i$, $f_j$, their similarity is computed following the method proposed by \cite{DBLP:conf/nips/Zelnik-ManorP04}:
\begin{equation}\label{eq:payoff}
\omega(i,j)=exp\left\lbrace-\frac{d(f_i,f_j)}{\sigma_{i}\text{ }\sigma_{j}}\right\rbrace
\end{equation}
where $d(f_i,f_j)$ denotes the similarity distance between features $f_i$ and $f_j$ and $\sigma_{i}$ corresponds to the distance between $i$ and its $7$-nearest- neighbors. Similarity values are stored in matrix $W$.

\paragraph{Finding Nash Equilibria}
The last component of our method is an algorithm for finding equilibrium conditions in this game. In \cite{DBLP:journals/neco/ErdemP12} a result from Evolutionary Game Theory \cite{weibull1997evolutionary}, named Replicator Dynamics (RD) \cite{smith1982evolution} is used. The RD are a class of dynamical systems that perform a natural selection process on a multi-population of strategies. The idea is to lead the fittest strategies to survive while the others to go extinct. More specifically the RD are defined as follow: 
\begin{equation}
x_i(h)^{t + 1} = x_i(h)^{t}\frac{u_i(h)^t}{u_i(x^t)}
\end{equation}
where $x_i(h)^{t}$ is the probability of strategy $h$ at time $t$ for player $i$.\\
The RD are iterated until convergence, this means either the distance between two successive steps is zero (formally $||x^{t+1}-x^t||_2 \leq \varepsilon$) or a certain amount of iterations is reached (See \cite{DBLP:journals/jmiv/Pelillo97} for a detailed analysis). In practical applications one could set the $\varepsilon$ to a small number but typically 10-20 iterations are sufficient.

%%%%%%%% END COPYPASTE ICPR %%%%%%%%%%%%%
